Artificial Intelligence: 70 Years Down the Road

Artificial intelligence (AI) has a history of nearly a century from its inception to the present day. We have summarized the development trends and discovered universal rules, including both success and failure. We have analyzed the reasons from both technical and philosophical perspectives to help understand the reasons behind the past failures and current successes of AI, and to provide a basis for thinking and exploring future development. Specifically, we have found that the development of AI in different fields, including computer vision, natural language processing, and machine learning, follows a pattern from rules to statistics to data-driven methods. In the face of past failures and current successes, we need to think systematically about the reasons behind them. Given the unity of AI between natural and social sciences, it is necessary to incorporate philosophical thinking to understand and solve AI problems, and we believe that starting from the dialectical method of Marx is a feasible path. We have concluded that the sustainable development direction of AI should be human-machine collaboration and a technology path centered on computing power. Finally, we have summarized the impact of AI on society from this trend.

==> tex/3_Intelligence.tex <==

\section{The Future of AI}


Essentially, artificial intelligence simulates the human thinking process from intuitive to rational cognition, so understanding the actual human thinking process is fundamental to artificial intelligence. Artificial intelligence mechanizes and mathematizes a part of the actual human thinking process. However, in the past, we focused on conceptual deduction of this thinking process, such as Marr's visual process and Saussure's language symbols mentioned in Chapter 2. They abstracted this thinking process, but these abstractions were proven to be incorrect in long-term practice. Therefore, we need to constantly verify the actual thinking process we propose in practice, which is the fact deduction of Marxist dialectics. Human-machine cooperation is the inevitable result of this philosophical idea in artificial intelligence. ChatGPT uses reinforcement learning for human-machine collaboration, and iterates the model based on human preferences, which is a very successful attempt.

Artificial intelligence must be based on human-machine cooperation, rather than unilateral machine intelligence. First, we need to answer: what can humans do and what can they not do? The human brain can use conceptual thinking to process experience and generate new knowledge, but the data that the human brain can handle is limited. Regarding computers, we need to answer: what can machines do and what they cannot do? We all know that machines can calculate efficiently, and anything that can be calculated can be done using computers. However, machines themselves cannot discern the truth of knowledge and may even forge knowledge.

Based on this, the efforts needed for artificial intelligence include: 1. improving computable boundaries; 2. enhancing computing power; 3. human feedback. Regarding the first one, the importance of mathematics is self-evident, but we also need to emphasize the importance of data. Computable boundaries can be promoted through data-driven methods, which is the experience gained from the past successful practices of AI. Especially in cases where mathematical tools are limited, data can be infinite, which can compensate for the inadequacy of mathematical tools. Regarding the second one, it requires contributions from multiple disciplines, including the development of physical theory, chip manufacturing capabilities, and sustainable energy. As for the third one, we need to solve the problem of how to feed back the complex thinking process of humans to machines, because most of the thinking processes cannot be quantified by simple sorting like ChatGPT, in order to complete the transfer.




==> tex/ack.tex <==
% \section{Acknowledgement}



\paragraph{ \bf Afterword and Acknowledgement}





\paragraph{Contribution.}
This paper 



==> tex/future.tex <==

\section{Future }
